TOI 560 : Two Transiting Planets Orbiting a K Dwarf Validated with iSHELL, PFS and HIRES RVs

We validate the presence of a two-planet system orbiting the 0.15--1.4 Gyr K4 dwarf TOI 560 (HD 73583). The system consists of an inner moderately eccentric transiting mini-Neptune (TOI 560 b, $P = 6.3980661^{+0.0000095}_{-0.0000097}$ days, $e=0.294^{+0.13}_{-0.062}$, $M= 0.94^{+0.31}_{-0.23}M_{Nep}$) initially discovered in the Sector 8 \tess\ mission observations, and a transiting mini-Neptune (TOI 560 c, $P = 18.8805^{+0.0024}_{-0.0011}$ days, $M= 1.32^{+0.29}_{-0.32}M_{Nep}$) discovered in the Sector 34 observations, in a rare near-1:3 orbital resonance. We utilize photometric data from \tess\, \textit{Spitzer}, and ground-based follow-up observations to confirm the ephemerides and period of the transiting planets, vet false positive scenarios, and detect the photo-eccentric effect for TOI 560 b. We obtain follow-up spectroscopy and corresponding precise radial velocities (RVs) with the iSHELL spectrograph at the NASA Infrared Telescope Facility and the HIRES Spectrograph at Keck Observatory to validate the planetary nature of these signals, which we combine with published PFS RVs from Magellan Observatory. We detect the masses of both planets at $> 3-\sigma$ significance. We apply a Gaussian process (GP) model to the \tess\ light curves to place priors on a chromatic radial velocity GP model to constrain the stellar activity of the TOI 560 host star, and confirm a strong wavelength dependence for the stellar activity demonstrating the ability of NIR RVs in mitigating stellar activity for young K dwarfs. TOI 560 is a nearby moderately young multi-planet system with two planets suitable for atmospheric characterization with James Webb Space Telescope (JWST) and other upcoming missions. In particular, it will undergo six transit pairs separated by $<$6 hours before June 2027.

==> measurements.tex <==
\begin{table*}[]
    \centering
    \begin{tabularx}{\textwidth}{@{\extracolsep{\fill}}XXXXX}
        \hline
        \hline
        Instrument / Facility & $N_{\rm transits}$ & Filter & Plate Scale & Precision \\
        \hline
        TESS & 7 & TESS & $\angd{;;22}\, {\rm px}^{-1}$ & $1 \times 10^{-3}$\\
        NGTS / Paranal & 1 & NGTS & $\angd{;;5}\, {\rm px}^{-1}$ & $1 \times 10^{-2}$ \\
        CTIO 1 m / LCO & 1 & $z'$ & $\angd{;;0.389}\, {\rm px}^{-1}$ & $8 \times 10^{-4}$ \\
        TMMT / LCO & 1 & I & $\angd{;;1.19}\, {\rm px}^{-1}$ & $2 \times 10^{-3}$ \\
        MuSCAT2 / TCS & 4 & $g'$, $i'$, $r'$, $z'$ & $\angd{;;0.44}\, {\rm px}^{-1}$ & $2 \times 10^{-3}$ \\
        KeplerCam / FLWO & 1 & B & $\angd{;;0.672}\, {\rm px}^{-1}$ & $2 \times 10^{-3}$ \\
        LCRO / LCO & 1 & $i'$ & $\angd{;;0.773}\, {\rm px}^{-1}$ & $4 \times 10^{-3}$ \\
    \end{tabularx}
    
    \begin{tabularx}{\textwidth}{@{\extracolsep{\fill}}XXXX}
        \hline
        \hline
        Instrument / Facility & UT Observation Dates & Wavelength & Separation Range \\
        \hline
        \textit{Zorro} / Gemini South & 2020-03-16 & 562 nm, 832 nm & $\angd{;;0.02}$--$\angd{;;1.2}$ \\
        NIRC2 / Keck II & 2019-05-12 & Br$\gamma$ & $\angd{;;0.02}$--$\angd{;;4}$ \\
        NIRI / Gemini North & 2019-05-23 & Br$\gamma$ & $\angd{;;0.02}$--$\angd{;;7}$ \\
        NESSI / WIYN & 2019-11-09 & 562 nm, 832 nm & $\angd{;;0.04}$--$\angd{;;1.2}$\\
        ShaneAO / Lick & 2021-02-26, 2021-02-27 & Ks, J & $\angd{;;0.6}$--$\angd{;;7}$ \\
    \end{tabularx}
    
    \begin{tabularx}{\textwidth}{@{\extracolsep{\fill}}llXXXXl}
        \hline
        \hline
        Instrument / Facility & $\lambda$ [\AA] & $\lambda / \Delta\lambda$ $[\times 10^{3}]$ & $N_{\rm nights}$ & $N_{\rm used}$ & $\sigma_{\rm RV}$ [\ms] & Pipeline \\
        \hline
        iSHELL / IRTF & 10600--53000 & 85 & 34 & 31 & 5.3 & \texttt{pychell} \citep{Cale2019} \\
        CARMENES-Vis / Calar Alto & 5200--9000 & 94.6 & 7 & 6 & 1.7 & \texttt{serval} \citep{zechmeister2018} \\
        CARMENES-NIR / Calar Alto & 9600--17100 & 80.4 & 7 & 7 & 7.2 & \texttt{serval} \citep{zechmeister2018} \\
        MAROON-X blue / Gemini North & 5000--6780 & 85 & 8 & 8 & 2.3 & \texttt{serval} \citep{zechmeister2018} \\
        MAROON-X red / Gemini North & 6540--9200 & 85 & 8 & 8 & 1.9 & \texttt{serval} \citep{zechmeister2018} \\
        NEID / WIYN & 4580--8920 & 120 & 8 & 8 & 1.1 & \texttt{serval} \citep{zechmeister2018} \\
        TRES / Tillinghast & 3850--9096 & 44 & 2 & 2 & -- & -- \\
        \hline
    \end{tabularx}
    \caption{Summary of all transit, high-contrast imaging, and radial velocity observations used in this work.  In the transit column headings, $N_{\rm transits}$ denotes the number of transits observed by that instrument and Precision denotes the order of magnitude of the normalized flux error for each instrument.  In the RV column headings, $N_{\rm nights}$ and $N_{\rm used}$ refer to the number of nights gathered and the number used, respectively.  The median intrinsic error bars $\sigma_{\rm RV}$ are calculated using only the nights used.}
    \label{tab:measurement_table}
\end{table*}
